Efficient Trace Encodings of Bounded Synthesis for Asynchronous Distributed Systems

The manual implementation of distributed systems is an error-prone task because of the asynchronous interplay of components and the environment. Bounded synthesis automatically generates an implementation for the specification of the distributed system if one exists. So far, bounded synthesis for distributed systems does not utilize their asynchronous nature. Instead, concurrent behavior of components is encoded by all interleavings and only then checked against the specification. We close this gap by identifying true concurrency in synthesis of asynchronous distributed systems represented as Petri games. This defines when several interleavings can be subsumed by one true concurrent trace. Thereby, fewer and shorter verification problems have to be solved in each iteration of the bounded synthesis algorithm. For Petri games, experimental results show that our implementation using true concurrency outperforms the implementation based on checking all interleavings.

==> InputFigures/QBFTrueConcurrent.tex <==
% !TeX root = ../Paper.tex
	The true concurrent encoding of bounded synthesis for Petri games formally replaces $\mathit{onetransition}_i$ of Appendix~\ref{appendix:seqEncoding} with $\mathit{trueconcurrentflow}_i$:
	\begin{eqnarray*}
	 	\mathit{trueconcurrentflow}_{i} & \defEQ & \big( \bigwedge_{\cpset_j \in \setcpsetsB} \neg \mathit{isenabled}_{i,{\cpset_j}} \wedge \mathit{fireonetransition}_{i,\tr^b}\big) \\
	 	&& \vee \big(\bigvee_{\cpset_j \in \setcpsetsB} \mathit{isenabled}_{i,{\cpset_j}} \wedge \bigwedge_{\cpset_j \in \setcpsetsB} \mathit{decision}_{i,\cpset_j} \big)\\
	 	\mathit{isenabled}_{i,\cpset_j} & \defEQ & \bigwedge_{p \in \pre{}{\cpset_j} } (p,i)   \wedge  \bigvee_{t \in \cpset_j} \  \bigwedge_{ p \in \pre{}{\cpset_j}\cap \plS^b} (p, \lambda^b(t))\\
	 	\mathit{decision}_{i, \cpset_j} & \defEQ & (\mathit{fire}_{i,\cpset_j}) \vee (\mathit{donotfire}_{i,\cpset_j})\\
	 	\mathit{fire}_{i,\cpset_j} & \defEQ & \mathit{isenabled}_{i,\cpset_j} \wedge \mathit{fireonetransition}_{i,\cpset_j}\\
	 	\mathit{fireonetransition}_{i,S} & \defEQ & \bigvee_{t \in S} \Big( \big(\bigwedge_{p \in \pre{}{t}} (p,i) \big) \wedge \big( \bigwedge_{p \in \pre{}{t}\cap \plS^b} (p, \lambda(t))\big) \\  
	 	&&\wedge \big( \bigwedge_{p \in \post{}{t}} (p, i+1) \big) 
	 	\wedge \big( \bigwedge_{p \in \pre{}{S} \setminus{(\pre{}{t}\cup \post{}{t})}} (p,i) \Leftrightarrow (p,i+1) \big) \\ 
	 	&&\wedge  \big( \bigwedge_{p \in \pre{}{t}{\setminus \post{}{t}}} \neg(p, i+1) \big)\\
	 	\mathit{donotfire}_{i,\cpset_j} & \defEQ & \neg \mathit{isenabled}_{i,\cpset_j} \wedge \bigwedge_{p \in \pre{}{\cpset_j}} (p,i) \Rightarrow  (p,i+1) \\
	 	&& \wedge \bigwedge_{p \in \post{}{\cpset_j}} \big( \bigvee_{\cpset_l \in \setcpsetsB, p \in \post{}{\cpset_l}, \cpset_j \neq \cpset_l} \mathit{isenabled}_{i,\cpset_l}\vee \neg (p,i) \Rightarrow \neg (p,i+1) \big)
 	\end{eqnarray*}

==> InputFiles/Proof.tex <==
% !TeX spellcheck = en_GB

% !TeX root = ../Paper.tex
In this section, we prove that the true concurrency firing semantics introduced in Section \ref{sec:trueconcurrencyfiringsemantics} and the sequential firing semantics are equivalent with respect to the avoidance of bad places in strategies for finite unfoldings of Petri games. 

\subsection{Traces}
We will show that every behavior of players in the Petri game defined by the sequential flow can be simulated with the true concurrent flow and vice versa. 
To formalize the behavior of all players in an unfolded game, we introduce traces of finite runs and their reached markings.
Recall that in a run, all choices of players have been resolved by deleting transitions and their following nodes.
\begin{definition}{\emph{(Sequential trace)}}
	\makebox[30mm][r]{}\\
	A \emph{sequential, finite, initial trace}  $\seqtrace = \langle t_1,\ldots,t_n \rangle$ with  $\init \firable{t_1} M_1 \firable{t_2}\ldots\firable{t_n} M_n = M_{\seqtrace}$ is a finite sequence of transitions that are fired on an initial run~$\run$ of a Petri game~$\pGame$.
\end{definition}

We call $M_{\seqtrace}$ the \emph{reached marking} of the trace $\trace$. For the  places in the visited markings of the trace, it holds that: ${\forall p\in \init\cup M_1\cup \ldots\cup M_n : |\post{}{p}| \leq 1}$.

% TODO only pairwise
We define reordering for sequential traces.
\begin{definition}{\emph{(Reordered traces)}}
	\makebox[30mm][r]{}\\
	For a sequential trace $\seqtrace = \langle t_1,\ldots,t_n\rangle$, a sequential trace $\reorderedtrace = \langle t_1^r,\ldots, t_i^r\rangle$ on the same initial run~$\run$ of a Petri game~$\pGame$ is a \emph{reordered, finite, initial trace} iff $\exists i\in\{1,\ldots, n-1\} : t_1 = t_1^r \wedge \ldots \wedge t_{i-1} = t_{i-1}^r \wedge t_i = t_{i+1}^r \wedge t_{i + 1} = t_{i}^r \wedge t_{i+2} = t_{i+2}^r \wedge \ldots \wedge t_n = t_n^r $.
	\label{def:reorderedruns}
\end{definition}

Notice that except for $M_i$ and $M_i^r$, the markings along the traces $\seqtrace$ and $\seqtrace^r$ are the same including the reached markings.

% TODO equivalence, equivalence relation etc needs to be way clearer
The reordering relation is an equivalence relation. Reordering the transitions of a trace such that the behavior of tokens does not change and the semantics of the Petri game is still satisfied gives us the possibility to modify the firing order of transitions that are enabled at the same marking. 

In a true concurrent trace, between two subsequent markings a set of tc-enabled transitions is fired. 
If every set of transitions in $\tctrace$ contains only one transition each, then it represents a sequential trace. 
Notice that the sets of transitions in $\tctrace$ do not provide an order of their transitions, but only an order of cp-sets. 
In sequential traces, some transitions can be reordered. 
Next, we will give a condition based on true concurrent traces when exactly this is the case.

% TODO somulate same behavior needs to be way clearer
To deploy reordered traces in our correctness proof of the true concurrency flow, we state the following:
\begin{theorem}{\emph{(Substituting reordered traces)}}
	\makebox[30mm][r]{}\\
	A sequential trace $\seqtrace$ and every reordered trace~$\seqtrace^r$ agree on the reaching of bad places, i.e., $\seqtrace$ reaches a bad place iff $\seqtrace^r$ reaches a bad place.
	\label{th:substitutingruns}
\end{theorem}
\begin{proof}
	For the length of the two traces $n$, let $i \in \{1,\ldots,n-1\}$ be the index of the difference between the two traces. 
	By definition, the markings are the same for all other indexes. Let $M_i$ and $M_i^r$ be the different reached markings after firing $t_i ( = t_{i+1}^r)$ and $t_i^r (= t_{i+1})$, respectively. 
	We show that the reached places $M_{i-1} \cup M_i \cup M_{i+1}$ and $M_{i-1}^r \cup M_i^r \cup M_{i+1}^r$ are the same.
	Notice that $M_{i-1} = M_{i-1}^r$ and $M_{i+1} = M_{i+1}^r$.
	The markings of index $i+1$ contain the places in the postset of both reordered transitions whereas the different markings contain only the places from the postset of one transition.
	Therefore, the same places are reached when reordering and both traces also agrees on the reaching of bad places.
	\qed
	\label{ProofReordering}
\end{proof}

We lift this definition to true concurrent flows and define true concurrent traces and their reached markings.
\begin{definition}{\emph{(True concurrent trace)}}	\makebox[30mm][r]{}\\
	A \emph{true concurrent, finite, initial trace} $\tctrace = \big\langle \{ t_{1,1},...,t_{n_1,1} \},\ldots,\{ t_{1,i},...,t_{n_i,i}\} \big\rangle$ with $\mathit{In} \firable{\{t_{1,1},...,t_{n_1,1}\}} M_1 \firable{\{t_{1,2}, ... , t_{n_2,2}\}} \ldots \firable{\{t_{1,i},...,t_{n_i,i}\}} M_i = M_{\tctrace}$ and all $n_1,...,n_i$ greater than 0 is a finite sequence of sets of tc-enabled transitions that are fired on an initial run~$\run$ of a Petri game $\pGame$.
		\label{def:trueconcurrentrun}
\end{definition}

We call $M_{\tctrace}$ the reached marking of the true concurrent trace $\tctrace$. For the places in the visited markings of the trace, it holds that: $\forall p\in \init\cup M_1\cup \ldots\cup M_i : |\post{}{p}| \leq 1$.


\subsection{Equivalence of Traces}
To prove the equivalence of the true concurrent flow and the sequential flow, we state the following:
\begin{theorem}{\emph{(Equivalence)}}
	\makebox[30mm][r]{}\\
	For every \textit{true concurrent} trace of a Petri game $\pGame$, there exists a \textit{transformed sequential} trace of the game, that the true concurrent trace can be transformed into. For every \textit{sequential} trace of the game, there exists a reordered sequential trace that can be transformed into a \textit{true concurrent} trace.
	\label{th:transformingruns}
\end{theorem}

We define a syntactic transformation from true concurrent traces to sequential traces and vice versa to be able to establish our equivalence theorem. We use the notation $\pGame[\markingPG]$ for a Petri game $\pGame$ with initial marking $\init = \markingPG$.
\begin{definition}{\emph{(Transforming Traces)}}
	\makebox[30mm][r]{}
	\begin{itemize}
		\item [$\Rightarrow$] $\tctrace$ to $\trace$:
		We transform $\tctrace = \big\langle \{ t_{1,1},...,t_{n_1,1} \} , \ldots , \{ t_{1,i},...,t_{n_i,i}\} \big\rangle$ to \\$\trace = \langle t_{1,1},...,t_{n_1,1}, ... ,t_{1,i},...,t_{n_i,i}\rangle$ by unrolling the sets of transitions to a sequence of ordered transitions subsequently. 
		\item [$\Leftarrow$] $\trace$ to $\tctrace$:
		 We need two steps to transform the sequential trace to a corresponding true concurrent trace:
		 \begin{enumerate}
		 	\item For all $t_i, t_{i+1}$ in $\trace$ where $t_i$ is only \emph{enabled} at marking $\pGame[\markingPG_{i-1}]$ and $t_{i+1}$ is \emph{tc-enabled} at $\pGame[M_{i-1}]$, change the order of $t_i$ and $t_{i+1}$.
		 	\item Build maximal sets of the transitions of the reordered trace such that all transitions $t_i, \ldots,t_j$ that are tc-enabled at $\pGame[\markingPG_{i-1}]$ belong to the same set. We build $\tctrace$ with the tuples in the respective order. 
		 \end{enumerate}
	\label{def:simulatingruns}
	\end{itemize}
\end{definition}
The proof of correctness for Definition~\ref{def:simulatingruns} and Theorem~\ref{th:transformingruns} can be found in Appendix~\ref{appendix:proofTransformingRuns}.


With the definition of reordered traces, we construct equivalence classes of traces that deliver the same history of tokens and result of the game and can therefore be reduced to one of the traces of each class. We restrict the possible traces to the tc-traces and therefore the \textit{reachable} markings of the game invalidating the behavior of tokens in the Petri game. Notice that true concurrent firing semantics is only applicable to Petri games that define their winning condition with \textit{bad places} and not \textit{bad markings}. Since we reduce the number of reachable markings, we could skip bad markings and therefore invalidate the game.

The proof shows the correctness of the introduced true concurrency firing semantics depending on the sequential firing semantics. Our proof is based on infinite unfoldings which are not applicable for our implementation. We therefore have to define traces for \textit{bounded unfoldings} and \textit{bounded runs}. 

\subsection{Bounded Traces}
If we consider \textit{bounded unfoldings} of a Petri game, at some point in the flow we reach a visited marking again. As explained before, we lose the causal history of the tokens in this marking since we cannot differentiate between both visits. This behavior is observed by a loop or by reaching the initial marking again which is a special case of a loop since we reach a marking that has been visited before. 

Traces as defined beforehand implicitly avoid losing the causal history. Since we define the postset and preset of places to a maximum of one transition, even reaching the same marking again, which corresponds to a loop, has a distinct causal past. Whenever a previously visited marking occurs, all following transitions are repetitions of previous sub tuples of the trace to the repeating marking. With that intuition we define \textit{bounded traces}:
\begin{definition}{(Bounded Traces)}
	\makebox[30mm][r]{}\\
	For a bounded unfolding of a Petri game, a  \textit{bounded} sequential trace $\boundedtrace = \langle t_1, \ldots, t_i \rangle$ with  $\mathit{In} [t_1\rangle M_1 [t_2\rangle \ldots [t_i\rangle M_i$ is a sequence of transitions that are fired, where either $\exists^{\leq 1} \ M_j. \ 0 \leq j \leq i-1. \ M_j = M_i$ and no other markings are equal or all markings are unique. 
	\label{def:boundedruns}
\end{definition}
The definition of bounded \textit{true concurrent} traces is synchronous to Definition \ref{def:boundedruns} and Definition \ref{def:trueconcurrentrun}. 
With the newly introduced \textit{bounded traces}, we avoid multiple occurrences of  transitions in  traces and can apply Proof \ref{ProofReordering} and the proof in Appendix \ref{ProofEquivalence} to these traces and bounded unfoldings.
We proved the correctness of our true concurrent firing approach on infinite unfoldings and bounded unfoldings of Petri games. Since the initial Petri game is equivalent to its unfolding with bound 1 for all places, we can apply our true concurrent flow also to non unfolded games.  





 	

==> InputFiles/ProofTransformingRuns.tex <==
% !TeX root = ../Paper.tex
\label{appendix:ProofTransformingRuns}
\begin{proof}
	We prove the Theorem \ref{th:transformingruns} and with it, that we can simulate true concurrent flow sequentially and vice versa.\\
	
	We claim that for all true concurrent traces $\tctrace$ there exists a sequential trace $\trace$ we can transform $\tctrace$ into and for all sequential traces $\trace$ there exists a reordered sequential trace $\reorderedtrace$ that can be transformed to a true concurrent trace $\tctrace$. 
	\begin{enumerate}
		\item[$''\Rightarrow''$] \textbf{$\forall \tctrace \exists \trace$ that can be transformed from  $\tctrace$}
		We use the construction given in Definition \ref{def:simulatingruns}. We know that if the construction is correct and universally applicable, then we find a simulating trace by transforming $\tctrace$ to the trace $\trace$. The transformation is based on firing the transitions of a set in $\tctrace$ sequentially, so we show that this is possible and does not invalidate the semantics of a Petri game, which is the behavior of the tokens in the game.\\
		Since all transitions in one set of the tuple corresponding to $\tctrace$ are in different transition sets by definition, firing them in any order will not change the \textit{enabledness} of each other. After firing the set corresponding to the $i$'th element of the tuple with $j$ transitions sequentially, we know that the marking $\markingPG_{i+j}$ in the sequential trace transformed up to this point enables all transitions in the following set of the true concurrent run and we can fire them again. With that, the transformation is correct and delivers a sequential run for every true concurrent run, where the causal past of all tokens in the reached marking did not change.
		\item[$''\Leftarrow''$] \textbf{$\forall \trace \exists \reorderedtrace$ that can be transformed to run $\tctrace$.}
		
		We adjust the order of the transitions of the trace as defined in Definition  \ref{def:simulatingruns}. With that we create a reordered run that can be directly transformed to a true concurrent run $\pi_C$ and show that the transformation is correct.\\
		\begin{enumerate}
			\item[\textbf{Step 1}] We start at $t_1$. For all pairs of transitions $t_i, t_{i+1}$ and corresponding markings $M_{i-1},M_{i}$, if $\pGame[M_{i-1}]$ enables $t_i$ sequentially and the cp-set of $t_{i+1}$ true concurrently, we switch the order of transition $t_{i-1}$ and $t_{i}$. We apply this reordering until no transitions can be switched. Since both transitions are independent, changing the firing order does not affect the causal past and result of the game.
			\item [\textbf{Step 2}] (a) If $t_i$ is tc-enabled at $\pGame[M_{i-1}]$, we take all following $j$ transitions where the corresponding cp-set is tc-enabled at $\pGame[M_{i-1}]$, until a only sequentially enabled transition is found. With all found transitions we build the set $\{t_{1,i},...,t_{j,i}\}$ and continue at $t_{j-1}$ and $M_j$ again with (a). Since all transitions in the set are mutual exclusive, firing them in one iteration step does not affect the game.\\
			(b) If $t_i$ is not true concurrently enabled at $M_{i-1}$, we build the one elementary set $\{t_i\}$ and go to $t_i+1$ starting step 2 again.
		\end{enumerate}
		The transformed reordered tuple with sets is exactly the transformed true concurrent run of $\trace$. The transformation steps simulate the true concurrent flow, since true concurrently enabled sets are fired first and all simultaneously enabled sets are fired in one step. This is exactly the definition of the true concurrency flow in Definition \ref{def:trueconcurrentflow}.
	\end{enumerate}
	Since both directions have been proven, we can say that for an arbitrary Petri game the sequential flow and the true concurrent flow simulate the same behavior of tokens in the game. They can be substituted without losing information or changing the result of a run and therefore the Petri game.\\
	\qed
\end{proof}

==> InputFiles/RunningExampleEasy.tex <==
% !TeX root = ../Paper.tex
	\begin{figure}
		\label{fig:RunningExampleEasy}
	\captionsetup[subfigure]{font=footnotesize}
	\centering
	
	
	\begin{tikzpicture}
	%Gobal Flow places
	\node [envplace] (env) [tokens = 1, label=above:\textit{Env}]{};

	
	\node [envplace] (e1) [left of = env, left of=env, left of = env, below of = env, below of = env, below of = env, label=left:\textit{e1}]{};
	\node [envplace] (e2) [right of=env, right of = env,right of = env,below of = env, below of = env, below of = env, label=right:\textit{e2}]{};
	\node [sysplace] (s1) [tokens = 1, right of = e1, label=right:\textit{s1}]{};
	\node [sysplace] (s2) [tokens = 1, left of = e2, label=left:\textit{s2}]{};
	
	\node [sysplace] (done11) [below of = s1, below of = s1, label =  right:\textit{done11}]{};
	\node [sysplace] (done12) [below of = s1, below of = s1,  left of = s1, label = left:\textit{done12}]{};
	\node [sysplace] (done21) [below of = s2, below of = s2,  label = left:\textit{done21}]{};
	\node [sysplace] (done22) [below of = s2, below of = s2,  right of = s2, label = right:\textit{done22}]{};
	
	%Bad behaviour check places
	\node [sysplace] (tcheck1) [left of= env, left of= env,left of = env, below of = env, label=left:\textit{1\_sub\_check}]{};

	\node [sysplace] (tcheck2) [right of= env, right of= env, right of = env, below of = env, label=right:\textit{2\_sub\_check}]{};

	
	%Syscheck for right decision of systems:
	
	\node [sysplace, bad] (bad) [below of = done11, below of = done11, right of = done11,  right of = done11,label = below:\textit{bad}]{};
	
	%Flow transitions
	\node [transition](t1) [below of= env, left of= env, label=above left:\textit{1\_subp}]{};
	\node [transition](t2) [below of= env,right of=env, label=above right:\textit{2\_subp}]{};
	
	
	\node [transition] (tdec11) [below of = s1, label =  right:\textit{dec1t}]{};
	\node [transition] (tdec12) [below of = s1, left of= s1, label = left:\textit{dec1f}]{};
	
	\node [transition] (tdec21) [below of = s2, label =  left:\textit{dec2t}]{};
	\node [transition] (tdec22) [below of = s2, right of= s2, label = right:\textit{dec2f}]{};
	
	
	%Bad behaviour transitions
	\node [transition] (tbad3) [ below of= done11, label = below left:\textit{badlocal1}]{};
	\node [transition] (tbad4) [ below of= done21, label = below right:\textit{badlocal2}]{};
	
	
	
	
	
	%Flow paths
	\path[->, thick] (t1) 
	edge [pre]  (env)
	edge [post] (tcheck1)

	edge [post] (e1);
	
	\path[->, thick] (t2) 
	edge [pre]  (env)
	edge [post] (tcheck2)

	edge [post] (e1)
	edge [post] (e2);
	
	\path[->, thick] (tdec11) 
	edge [pre]  (e1)
	edge [pre] (s1)
	edge [post] (done11);
	
	\path[->, thick] (tdec12) 
	edge [pre]  (e1)
	edge [pre] (s1)
	edge [post] (done12);
	
	\path[->, thick] (tdec21) 
	edge [pre]  (e2)
	edge [pre] (s2)
	edge [post] (done21);
	
	\path[->, thick] (tdec22) 
	edge [pre]  (e2)
	edge [pre] (s2)
	edge [post] (done22);
	
	
	\path [->, thick] (tbad3)
	edge [pre] (done11)
	edge [pre, bend left,in = 90, out = 90] (tcheck1)
	edge [post] (bad);
	
	\path [->, thick] (tbad4)
	edge [pre] (done21)
	edge [pre, bend right,in = 270, out = 270] (tcheck2)
	edge [post] (bad);
	\end{tikzpicture}
	\caption{Simple version without global system decision }
\end{figure}

==> InputFiles/RunningExampleHard.tex <==
% !TeX root = ../Paper.tex
\begin{figure}[H]
		\label{fig:RunningExampleHard}
		\captionsetup[subfigure]{font=footnotesize}
		\centering
		
	
			\begin{tikzpicture}[scale=0.7,every node/.style={transform shape}]
			%Gobal Flow places
 			\node [envplace] (env) [tokens = 1, label=above:\textit{Env}]{};
			\node [sysplace] (sys) [below of=env, below of= env, below of=env, label=right:\textit{Sys}]{};
			
			\node [envplace] (e1) [left of=sys, left of = sys, label=left:\textit{e1}]{};
			\node [envplace] (e2) [right of=sys, right of = sys, label=right:\textit{e2}]{};
			\node [sysplace] (s1) [below of=sys, below of=sys, left of=sys, label=right:\textit{s1}]{};
			\node [sysplace] (s2) [below of=sys, below of=sys,  right of = sys, label=left:\textit{s2}]{};
			
			\node [sysplace] (done11) [below of = s1, below of = s1, left of = s1, label = right:\textit{done11}]{};
			\node [sysplace] (done12) [below of = s1, below of = s1, left of = s1, left of = s1, label = left:\textit{done12}]{};
			\node [sysplace] (done21) [below of = s2, below of = s2, right of = s2, label = left:\textit{done21}]{};
			\node [sysplace] (done22) [below of = s2, below of = s2, right of = s2, right of = s2, label = right:\textit{done22}]{};
			
				%Bad behaviour check places
			\node [sysplace] (tcheck1) [left of= env, left of= env,left of = env, below of = env, label=left:\textit{1\_sub\_check}]{};
			\node [sysplace] (fcheck1) [below of = tcheck1, label=left:\textit{not\_2\_subp}]{};
			\node [sysplace] (tcheck2) [right of= env, right of= env, right of = env, below of = env, label=right:\textit{2\_sub\_check}]{};
			\node [sysplace] (fcheck2) [below of = tcheck2, label=right:\textit{not\_3\_subp}]{};
			
			%Syscheck for right decision of systems:
			\node [sysplace] (syscheck1) [left of= s1, left of = s1, left of = s1, label = left:\textit{s2check}]{};
			\node [sysplace] (syscheck2) [right of= s2, right of = s2, right of = s2, label = left:\textit{s1check}]{};
			
			\node [sysplace, bad] (bad) [below of = done11, below of = done11, right of = done11, right of = done11, label = below:\textit{bad}]{};
			\node [sysplace, bad] (badleft) [left of = e1,left of = e1, left of = e1, left of = e1, left of= e1,label = below:\textit{bad}]{};
			\node [sysplace, bad] (badright) [right of = e2, right of = e2, right of= e2, right of=e2,right of=e2, label = below:\textit{bad}]{};
			
			%Flow transitions
			\node [transition](t1) [below of= env, left of= env, label=above left:\textit{1\_subp}]{};
			\node [transition](t2) [below of= env,right of=env, label=above right:\textit{2\_subp}]{};
			
			\node [transition](t3) [below of= sys, left of= sys, label=above left:\textit{init\_1}]{};
			\node [transition](t4) [below of= sys, right of=sys, label=above right:\textit{init\_2}]{};
			
			\node [transition] (tdec11) [below of = s1,left of = s1, label = right:\textit{dec1t}]{};
			\node [transition] (tdec12) [below of = s1,left of = s1, left of= s1, label = left:\textit{dec1f}]{};
			
			\node [transition] (tdec21) [below of = s2,right of = s2, label = left:\textit{dec2t}]{};
			\node [transition] (tdec22) [below of = s2,right of = s2, right of= s2, label = right:\textit{dec2f}]{};
			
			
			%Bad behaviour transitions
			\node [transition] (tbad1) [right of = badleft, right of = badleft, label = below:\textit{badsys1}]{};
			\node [transition] (tbad2) [left of = badright, left of = badright, label = below:\textit{badsys2}]{};
			
			\node [transition] (tbad3) [ below of= done11, label = below left:\textit{badlocal1}]{};
			\node [transition] (tbad4) [ below of= done21, label = below right:\textit{badlocal2}]{};
			
			%Flow paths
			\path[->, thick] (t1) 
			edge [pre]  (env)
			edge [post]  (sys)
			edge [post] (tcheck1)
			edge [post] (fcheck1)
			edge [post] (e1);
			
			\path[->, thick] (t2) 
			edge [pre]  (env)
			edge [post]  (sys)
			edge [post] (tcheck2)
			edge [post] (fcheck2)
			edge [post] (e1)
			edge [post] (e2);
			
			\path[->, thick] (t3) 
			edge [pre]  (sys)
			edge [post] (s1)
			edge [post] (syscheck2);
						
			\path[->, thick] (t4) 
			edge [pre]  (sys)
			edge [post] (s1)
			edge [post] (s2)
			edge [post] (syscheck1);
			
			\path[->, thick] (tdec11) 
			edge [pre]  (e1)
			edge [pre] (s1)
			edge [post] (done11);
			
			\path[->, thick] (tdec12) 
			edge [pre]  (e1)
			edge [pre] (s1)
			edge [post] (done12);
			
			\path[->, thick] (tdec21) 
			edge [pre]  (e2)
			edge [pre] (s2)
			edge [post] (done21);
			
			\path[->, thick] (tdec22) 
			edge [pre]  (e2)
			edge [pre] (s2)
			edge [post] (done22);
			
			\path [->, thick] (tbad1)
			edge [pre] (syscheck1)
			edge [pre] (fcheck1)
			edge [post] (badleft);
			
			\path [->, thick] (tbad2)
			edge [pre] (syscheck2)
			edge [pre] (fcheck2)
			edge [post] (badright);
			
			\path [->, thick] (tbad3)
			edge [pre] (done11)
			edge [pre, bend left,in = 90, out = 90] (tcheck1)
			edge [post] (bad);
			
			\path [->, thick] (tbad4)
			edge [pre] (done21)
			edge [pre, bend right,in = 270, out = 270] (tcheck2)
			edge [post] (bad);
			\end{tikzpicture}
		\caption{Local sub-processes with global system decision }
		\label{PNexample}
	\end{figure}
